Coreference Resolution as Query-based Span Prediction

In this paper, we present an accurate and extensible approach for the coreference resolution task. We formulate the problem as a span prediction task, like in machine reading comprehension (MRC): A query is generated for each candidate mention using its surrounding context, and a span prediction module is employed to extract the text spans of the coreferences within the document using the generated query. This formulation comes with the following key advantages: (1) The span prediction strategy provides the flexibility of retrieving mentions left out at the mention proposal stage; (2) In the MRC framework, encoding the mention and its context explicitly in a query makes it possible to have a deep and thorough examination of cues embedded in the context of coreferent mentions; and (3) A plethora of existing MRC datasets can be used for data augmentation to improve the model's generalization capability. Experiments demonstrate significant performance boost over previous models, with 87.5 (+2.5) F1 score on the GAP benchmark and 83.1 (+3.5) F1 score on the CoNLL-2012 benchmark.

==> figures/token_rep.tex <==
\begin{figure}[t!]
\centering
\setlength{\fboxsep}{0.9em}
\fbox{\parbox{0.9\linewidth}{
 \textbf{Original Passage}
 
\textbf{Paula Zahn}: Here's Erica Hill from Headline News. Hi Erica.

\textbf{Erica Hill}: Hi Paula... I 'm sure I 'll be hearing a little bit more about it all week.

\textbf{Paula Zahn}: Thanks Erica. see you a little bit later on. 

\textbf{Converted Tokens}

[\texttt{[CLS]}, \texttt{[SPEAKER]}, \texttt{Paula}, \texttt{Zahn}, \texttt{[SPEAKER]}, \texttt{Here}, \texttt{'}, \texttt{s}, \texttt{Erica}, \texttt{Hill}, \texttt{from}, \texttt{Head}, \texttt{\#\#line}, \texttt{News}, \texttt{.}, \texttt{Hi}, \texttt{Erica}, \texttt{.}, \texttt{[SPEAKER]}, \texttt{Erica}, \texttt{Hill}, \texttt{[SPEAKER]}, \texttt{Hi}, \texttt{Paula}, ..., \texttt{I}, \texttt{'}, \texttt{m}, \texttt{sure}, \texttt{I}, \texttt{'}, \texttt{ll}, \texttt{be}, \texttt{hearing}, \texttt{a}, \texttt{little}, \texttt{bit}, \texttt{more}, \texttt{about}, \texttt{it}, \texttt{all}, \texttt{week}, \texttt{.}, \texttt{[SPEAKER]}, \texttt{Paula}, \texttt{Zahn}, \texttt{[SPEAKER]}, \texttt{Thanks}, \texttt{Erica}, \texttt{.}, \texttt{see}, \texttt{you}, \texttt{a}, \texttt{little}, \texttt{bit}, \texttt{later}, \texttt{on}, \texttt{.}, \texttt{[SEP]]}

}}
\caption{An illustration of the token conversion.}
\label{fig:token}
\end{figure}
